Using Background Knowledge to Rank Itemsets

Assessing the quality of discovered results is an important open problem in data mining. Such assessment is particularly vital when mining itemsets, since commonly many of the discovered patterns can be easily explained by background knowledge. The simplest approach to screen uninteresting patterns is to compare the observed frequency against the independence model. Since the parameters for the independence model are the column margins, we can view such screening as a way of using the column margins as background knowledge. In this paper we study techniques for more flexible approaches for infusing background knowledge. Namely, we show that we can efficiently use additional knowledge such as row margins, lazarus counts, and bounds of ones. We demonstrate that these statistics describe forms of data that occur in practice and have been studied in data mining. To infuse the information efficiently we use a maximum entropy approach. In its general setting, solving a maximum entropy model is infeasible, but we demonstrate that for our setting it can be solved in polynomial time. Experiments show that more sophisticated models fit the data better and that using more information improves the frequency prediction of itemsets.

==> prel.tex <==
\section{Preliminaries and Notation}
\label{sec:prel}

We begin by presenting preliminary concepts and notations that will be used
throughout the rest of the paper.

A \emph{binary dataset} $D$ is a collection of $\abs{D}$ \emph{transactions},
binary vectors of length $N$. The set of all possible transactions $t$ is written 
as $\Omega$. The $i$th element of a random transaction is
represented by an \emph{attribute} $a_i$, a Bernoulli random variable. We
denote the collection of all the attributes by $A = \enset{a_1}{a_N}$. An
\emph{itemset} $X = \enset{x_1}{x_L} \subseteq A$ is a subset of attributes. We
will often use the dense notation $X = \iset{x_1}{x_L}$.

Given an itemset $X$ and a binary vector $v$ of length $L$, we use the notation
$p\fpr{X = v}$ to express the probability of $p\fpr{x_1 = v_1, \ldots, x_L =
v_L}$. If $v$ contains only 1s, then we will use the notation $p\fpr{X = 1}$.

Given a binary dataset $D$ we define $q_D$ to be an \emph{empirical
distribution},
\[
	q_D\fpr{A = v} = \abs{\set{t \in D \mid t = v}} / {\abs{D}}.
\]
We define the \emph{frequency} of an itemset $X$ to be $\freq{X} = q_D\fpr{X = 1}$.

